Measurement of branching fractions of charmless four-body $\Lambda_b^0$ and $\Xi_b^0$ decays

A search for charmless four-body decays of $\Lambda_{b}^{0}$ and $\Xi_{b}^{0}$ baryons with a proton and three charged mesons (either kaons or pions) in the final state is performed. The data sample used was recorded in 2011 and 2012 with the LHCb experiment and corresponds to an integrated luminosity of 3 fb$^{-1}$. Six decay modes are observed, among which $\Lambda_{b}^{0} \to pK^{-}\pi^{+}\pi^{-}$, $\Lambda_{b}^{0} \to pK^{-}K^{+}K^{-}$, $\Xi_{b}^{0} \to pK^{-}\pi^{+}\pi^{-}$ and $\Xi_{b}^{0} \to pK^{-} \pi^{+}K^{-}$ are established for the first time. Their branching fractions (including the ratio of hadronisation fractions in the case of the $\Xi_{b}^{0}$ baryon) are determined relative to the $\Lambda_{b}^{0} \to \Lambda_{c}^{+}\pi^{-}$ decay.

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 


==> abstract.tex <==
 A search for charmless four-body decays of $\Lambda_b^0$ and $\Xi_b^0$ baryons with a proton and three charged mesons (either kaons or pions) in the final state is performed. The data sample used was recorded in 2011 and 2012 with the LHCb experiment and corresponds to an integrated luminosity of 3 fb$^{-1}$. Six decay modes are observed, among which $\Lambda_b^0 \to pK^{-}\pi^{+}\pi^{-}$, $\Lambda_b^0 \to pK^{-}K^{+}K^{-}$, $\Xi_b^0 \to pK^{-}\pi^{+}\pi^{-}$ and $\Xi_b^0 \to pK^{-}\pi^{+} K^{-}$ are established for the first time. Their branching fractions (including the ratio of hadronisation fractions in the case of the $\Xi_b^0$ baryon) are determined relative to the $\Lambda_b^0 \to Lambda_c^{+} \pi^{-}$ decay.
  


==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script ./listsymbols

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash cleo} & \cleo & \texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero \\
\texttt{\textbackslash aleph} & \aleph & \texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal \\
\texttt{\textbackslash lthree} & \lthree & \texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern \\
\texttt{\textbackslash lhc} & \lhc & \texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash epem} & \epem & \texttt{\textbackslash muon} & \muon \\
\texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash tautau} & \tautau & \texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm \\
\texttt{\textbackslash ellp} & \ellp & \texttt{\textbackslash ellell} & \ellell & \texttt{\textbackslash neu} & \neu \\
\texttt{\textbackslash neub} & \neub & \texttt{\textbackslash neue} & \neue & \texttt{\textbackslash neueb} & \neueb \\
\texttt{\textbackslash neum} & \neum & \texttt{\textbackslash neumb} & \neumb & \texttt{\textbackslash neut} & \neut \\
\texttt{\textbackslash neutb} & \neutb & \texttt{\textbackslash neul} & \neul & \texttt{\textbackslash neulb} & \neulb \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pizs} & \pizs & \texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim \\
\texttt{\textbackslash pipm} & \pipm & \texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson \\
\texttt{\textbackslash rhoz} & \rhoz & \texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom \\
\texttt{\textbackslash rhopm} & \rhopm & \texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz & \texttt{\textbackslash Kstarzb} & \Kstarzb \\
\texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb & \texttt{\textbackslash Kstarp} & \Kstarp \\
\texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm & \texttt{\textbackslash Kstarmp} & \Kstarmp \\
\texttt{\textbackslash etaz} & \etaz & \texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz \\
\texttt{\textbackslash omegaz} & \omegaz &  \\
\end{tabular*}

\subsubsection{Heavy mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db & \texttt{\textbackslash DorDbar} & \DorDbar \\
\texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb & \texttt{\textbackslash Dp} & \Dp \\
\texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm & \texttt{\textbackslash Dmp} & \Dmp \\
\texttt{\textbackslash Dstar} & \Dstar & \texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz \\
\texttt{\textbackslash Dstarzb} & \Dstarzb & \texttt{\textbackslash Dstarp} & \Dstarp & \texttt{\textbackslash Dstarm} & \Dstarm \\
\texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp & \texttt{\textbackslash Ds} & \Ds \\
\texttt{\textbackslash Dsp} & \Dsp & \texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm \\
\texttt{\textbackslash Dsmp} & \Dsmp & \texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp \\
\texttt{\textbackslash Dssm} & \Dssm & \texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp \\
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb \\
\texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp \\
\texttt{\textbackslash Bcm} & \Bcm & \texttt{\textbackslash Bcpm} & \Bcpm &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash chiczero} & \chiczero & \texttt{\textbackslash chicone} & \chicone \\
\texttt{\textbackslash chictwo} & \chictwo & \texttt{\textbackslash OneS} & \OneS & \texttt{\textbackslash TwoS} & \TwoS \\
\texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS & \texttt{\textbackslash FiveS} & \FiveS \\
\texttt{\textbackslash chic} & \chic &  \\
\end{tabular*}

\subsubsection{Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Lz} & \Lz \\
\texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar & \texttt{\textbackslash Lambdares} & \Lambdares \\
\texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares & \texttt{\textbackslash Sigmaresbar} & \Sigmaresbar \\
\texttt{\textbackslash Sigmaresbarz} & \Sigmaresbarz & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Lc} & \Lc \\
\texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz \\
\texttt{\textbackslash Xibm} & \Xibm & \texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz \\
\texttt{\textbackslash Xibbarp} & \Xibbarp & \texttt{\textbackslash Xic} & \Xic & \texttt{\textbackslash Xicz} & \Xicz \\
\texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar & \texttt{\textbackslash Xicbarz} & \Xicbarz \\
\texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac & \texttt{\textbackslash Omegacbar} & \Omegacbar \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BRvis} & \BRvis & \texttt{\textbackslash BR} & \BR \\
\texttt{\textbackslash decay[2] \textbackslash decay\{\Pa\}\{\Pb \Pc\}} & \decay{\Pa}{\Pb \Pc} & \texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar & \texttt{\textbackslash Vud} & \Vud \\
\texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd & \texttt{\textbackslash Vus} & \Vus \\
\texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts & \texttt{\textbackslash Vub} & \Vub \\
\texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb & \texttt{\textbackslash Vuds} & \Vuds \\
\texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds & \texttt{\textbackslash Vuss} & \Vuss \\
\texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss & \texttt{\textbackslash Vubs} & \Vubs \\
\texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs &  \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}} & \unit{kg} &  \\
\end{tabular*}

\subsubsection{Energy and momentum}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevc} & \gevc \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\texttt{\textbackslash mevcc} & \mevcc &  \\
\end{tabular*}

\subsubsection{Distance and area}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst &  \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqvs} & \chisqvs & \texttt{\textbackslash chisqvtx} & \chisqvtx \\
\texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv & \texttt{\textbackslash gsim} & \gsim \\
\texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} & \texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} \\
\texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag & \texttt{\textbackslash PDF} & \PDF \\
\texttt{\textbackslash sPlot} & \sPlot &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt \\
\texttt{\textbackslash dpp} & \dpp & \texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash krad} & \krad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig & \texttt{\textbackslash moore} & \moore \\
\texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos & \texttt{\textbackslash powheg} & \powheg \\
\texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos & \texttt{\textbackslash roofit} & \roofit \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice & \texttt{\textbackslash urania} & \urania \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn &  \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbytes} & \kbytes & \texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash kbits} & \kbits \\
\texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash mbytes} & \mbytes \\
\texttt{\textbackslash mbps} & \mbps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash gbsps} & \gbsps \\
\texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbsps} & \gbsps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbpy} & \tbpy & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}



==> principles.tex <==
\section{General principles}

The main goal is for a paper to be clear. It should be as brief as
possible, without sacrificing clarity. For all public documents,
special consideration should be given to the fact that the reader will
be less familiar with \lhcb than the author.

Here follow a list of general principles that should be adhered to:
\begin{enumerate}

\item Choices that are made concerning layout and typography
  should be consistently applied throughout the document.

\item Standard English should be used (British rather than American)
  for LHCb notes and preprints. Examples: colour, flavour, centre,
  metre, modelled and aluminium. Words ending on -ise or -isation
  (polarise, hadronisation) can be written with -ize or -ization ending but should be consistent.
  The punctuation normally follows the closing quote mark of quoted text, 
  rather than being included before the closing quote.
  Footnotes come after punctuation. 
  Papers to be submitted to an American journal can be written in American
  English instead. Under no circumstance should the two be mixed.

\item Use of jargon should be avoided where possible. ``Systematics'' are ``systematic
  uncertainties'', ``L0'' is ``hardware trigger'', ``penguin'' diagrams
  are best introduced with an expression like ``electroweak loop (penguin) diagrams''.

\item It would be good to avoid using quantities that are internal jargon and/or 
  are impossible to reproduce without the full simulation, \ie\ instead of ``It is 
  required that $\chisqvtx<3$'', to say ``A good quality vertex is required''; 
  instead of ``It is required that $\chisqip>16$'', to say ``The track is 
  inconsistent with originating from a PV''; instead of ``A DLL greater 
  than 20 is required'' say to ``Tracks are required to be identified as kaons''.
  However, experience shows that some journal referees ask for exactly this 
  kind of information, and to safeguard against this, one may consider given 
  some of it in the paper, since even if the exact meaning may be LHCb-specific, 
  it still conveys some qualitative feeling for the significance levels required 
  in the varies steps of the analysis.   
 
\item Latex should be used for typesetting. Line numbering should be
  switched on for drafts that are circulated for comments.

\item The abstract should be concise, and not include citations or
  numbered equations, and should give the key results from the paper.

\item Apart from descriptions of the detector, the trigger and the
  simulation, the text should not be cut-and-pasted from other sources
  that have previously been published.

\item References should usually be made only to publicly accessible
  documents. References to LHCb conference reports and public notes
  should be avoided in journal publications, instead including the
  relevant material in the paper itself.

\item The use of tenses should be consistent. It is recommended to
  mainly stay in the present tense, for the abstract, the description
  of the analysis, \etc; the past tense is then used where necessary,
  for example when describing the data taking conditions.

\item It is recommended to use the passive rather than active voice:
  ``the mass is measured'', rather than ``we measure the mass''.
  Limited use of the active voice is acceptable, in situations where
  re-writing in the passive form would be cumbersome, such as for the
  acknowledgements.  Some leeway is permitted to accommodate different
  author's styles, but ``we'' should not appear excessively in the
  abstract or the first lines of introduction or conclusion.

\item A sentence should not start with a variable, a particle or an acronym.
 A title or caption should not start with an article. 

\item Incorrect punctuation around conjunctive adverbs and the use of 
dangling modifiers are the two most common mistakes of English grammar
in LHCb draft papers. If in doubt, read the wikipedia articles on 
conjunctive adverb and dangling modifier.  

\item When using natural units, at the first occurence of an energy unit
      that refers to momentum or a radius, add a footnote: ``Natural units
      with $\hbar=c=1$ are used throughout.'' Do this even when somewhere
      a length is reported in units of mm. It's not 100\% consistent, but
      most likely nobody will notice. The problem can be trivially avoided
      when no lengths scales in natural units occur, by omitting the 
      $\hbar$ from the footnote text.

\item Papers dealing with amplitude analyses and/or resonance parameters, 
      other than masses and lifetimes, should use natural units,
      since in these kind of measurements widths are traditionally 
      expressed in MeV and radii in GeV$^{-1}$. It's also the convention
      used by the PDG. 
\end{enumerate}


==> reference.tex <==
\section{References}
\label{sec:References}

References should be made using Bib\TeX~\cite{BibTeX}. A special style
\texttt{LHCb.bst} has been created to achieve a uniform
style. Independent of the journal the paper is submitted to, the
preprint should be created using this style. Where arXiv numbers
exist, these should be added even for published articles. In the PDF
file, hyperlinks will be created to both the arXiv and the published
version.

\begin{enumerate}

\item Citations are marked using square brackets, and the
  corresponding references should be typeset using Bib\TeX\ and the
  official \lhcb Bib\TeX\ style. An example is in
  Ref.~\cite{Sjostrand:2006za}.

\item For references with four or less authors all of the authors'
  names are listed~\cite{Majorana:1937vz}, otherwise the first author
  is given, followed by \etal. The \lhcb Bib\TeX\ style will
  take care of this.

\item The order of references should be sequential when reading the
  document. This is automatic when using Bib\TeX.

\item The titles of papers should in general be included. To remove
  them, change \texttt{\textbackslash
    setboolean\{articletitles\}\{false\}} to \texttt{true} at the top
  of this template.
  Note that the titles in \verb!LHCb-PAPER.bib! are in plain LaTex,
  in order to correspond to the actual title on the arXiv record.
  Some differences in style can thus be noticed with respect to the
  main text, for example particle names that use capital Greek letters
  are not slanted in the reference titles ($\Lambda$ vs \Lz)  

\item Whenever possible, use references from the supplied files
\verb!main.bib!, \verb!LHCb-PAPER.bib!, \verb!LHCb-CONF.bib!, and \verb!LHCB-DP.bib!.
These are kept up-to-date by the EB. If you see a mistake, do not edit these files,
but let the EB know. This way, for every update of the paper, you save
yourself the work of updating the references. Instead, you can just copy or
check in the latest versions of the \verb!.bib! files from the repository.   

\item For those references not provided by the EB, the best
  is to copy the Bib\TeX\ entry directly from
  \texttt{Inspire}. Often these need to be edited to get the 
  correct title, author names and formatting. 
  For authors with multiple initials, add a space between them (change \texttt{R.G.C.} to \texttt{R. G. C.}),
  otherwise only the first initial will be taken. 
  Also, make sure to eliminate unnecessary capitalisation.
  Apart from that, the title should be respected as much as possible
  (\eg do not change particle names to PDG convention nor introduce/remove factors of $c$).
  Check that both the arXiv and the journal index are clickable
  and point to the right article.

%\item Even if the basic formatting of the Bib\TeX\ entry is taken from
%  \texttt{Inspire}, all the data should be cross checked against the
%  journal. Often there are minor changes to author initials or
%  titles. In case of a difference between the preprint and the
%  journal, the bibliographic information from the journal should be
%  used.

\item The \texttt{mciteplus}~\cite{mciteplus} package is used
  to enable multiple references to show up as a single item in the
  reference list. As an example \texttt{\textbackslash
    cite\{Mohapatra:1979ia,*Pascoli:2007qh\}} where the \texttt{*}
  indicates that the reference should be merged with the previous
  one. The result of this can be seen in
  Ref.~\cite{Mohapatra:1979ia,*Pascoli:2007qh}. Be aware that the
  \texttt{mciteplus} package should be included as the very last item
  before the \texttt{\textbackslash begin\{document\}} to work
  correctly.

\item It should be avoided to make references to public notes and
  conference reports in public documents. Exceptions can be discussed
  on a case-by-case basis with the review committee for the
  analysis. In internal reports they are of course welcome and can be
  referenced as seen in Ref.~\cite{LHCb-CONF-2011-003} using the
  \texttt{lhcbreport} category. For conference reports, omit the
  author field completely in the Bib\TeX\ record.

\item To get the typesetting and hyperlinks correct for \lhcb reports,
  the category \texttt{lhcbreport} should be used in the Bib\TeX\
  file. See Refs.~\cite{LHCb-INT-2011-047, *LHCb-ANA-2011-078,
    *CERN-THESIS-2014-057, *LHCb-PROC-2014-017, *LHCB-TALK-2014-257}
  for some examples. It can be used for \lhcb documents in the series
  \texttt{CONF}, \texttt{PAPER}, \texttt{PROC}, \texttt{THESIS},
  \texttt{LHCC}, \texttt{TDR} and internal \lhcb reports. Papers sent
  for publication, but not published yet, should be referred with
  their \texttt{arXiv} number, so the \texttt{PAPER} category should
  only be used in the rare case of a forward reference to a paper.

\item Proceedings can be used for references to items such as the
  \lhcb simulation~\cite{LHCb-PROC-2011-006}, where we do not yet have
  a published paper.

\end{enumerate}

There is a set of standard references to be used in \lhcb that are
listed in Appendix~\ref{sec:StandardReferences}.


==> title.tex <==
Measurement of branching fractions of charmless four-body $\Lambda_b^0$ and $\Xi_b^0$ decays


==> typography.tex <==
\section{Typography}
\label{sec:typography}

The use of the Latex typesetting symbols defined in the file
\texttt{lhcb-symbols-def.tex} and detailed in the appendices of this
document is strongly encouraged as it will make it much easier to
follow the recommendation set out below.

\begin{enumerate}

\item \lhcb is typeset with a normal (roman) lowercase b.

\item Titles are in bold face, and usually only the first word is
  capitalised.

\item Mathematical symbols and particle names should also be typeset
  in bold when appearing in titles.

\item Units are in roman type, except for constants such as $c$ or $h$
  that are italic: \gev, \gevcc.  The unit should be separated from
  the value with a thin space (``\verb!\,!''),
  and they should not be broken over two lines.
  Correct spacing is automatic when using predefined units inside math mode: \verb!$3.0\gev$! $\to 3.0\gev$.
  Spacing goes wrong when using predefined units outside math mode AND forcing extra space:
  \verb!3.0\,\gev! $\to$ 3.0\,\gev or worse:   \verb!3.0~\gev! $\to$ 3.0~\gev. 

\item  If factors of $c$ are kept, they should be used both for masses and
  momenta, \eg $p=5.2\gevc$ (or $\gev c^{-1}$), $m = 3.1\gevcc$ (or $\gev c^{-2}$). If they are dropped this
  should be done consistently throughout, and a note should be added
  at the first instance to indicate that units are taken with $c=1$.

\item The \% sign should not be separated from the number that precedes it: 5\%, not 5 \%. 
A thin space is also acceptable: 5\,\%, but should be applied consistently throughout the paper.

\item Ranges should be formatted consistently. The recommendend form is to use a dash with no spacing around it: 
7--8\gev, obtained as \verb!7--8\gev!. 

\item Italic is preferred for particle names (although roman is
  acceptable, if applied consistently throughout).  Particle Data
  Group conventions should generally be followed: \Bd (no need for a
  ``d'' subscript), \decay{\Bs}{\jpsi\phi}, \Bsb,
  (note the long bar, obtained with \verb!\overline!, in contrast to the discouraged short \verb!\bar{B}! resulting in $\bar{B}$), \KS (note the
  uppercase roman type ``S''). 
This is most easily achieved by using the predefined symbols described in 
  Appendix~\ref{sec:listofsymbols}.
  Unless there is a good reason not to, the charge of a particle should be
  specified if there is any possible ambiguity 
  ($m(\Kp\Km)$ instead of $m(KK)$, which could refer to neutral kaons).

\item Decay chains can be written in several ways, depending on the complexity and the number of times it occurs. Unless there is a good reason not to, usage of a particular type should be consistent within the paper.
Examples are: 
$\Dsp\to\phi\pip$, with $\phi\to\Kp\Km$; 
$\Dsp\to\phi\pip$ ($\phi\to\Kp\Km$);  
$\Dsp\to\phi(\to\Kp\Km)\pip$; or
$\Dsp\to[\Kp\Km]_\phi\pip$.



\item Variables are usually italic: $V$ is a voltage (variable), while
  1 V is a volt (unit). Also in combined expressions: $Q$-value, $z$-scale, $R$-parity \etc

\item Subscripts and superscripts are roman type when they refer to a word (such as T
  for transverse) and italic when they refer to a variable (such as
  $t$ for time): \pt, \dms, $t_{\mathrm{rec}}$.

\item Standard function names are in roman type: \eg $\cos$, $\sin$
  and $\exp$.

\item Figure, Section, Equation, Chapter and Reference should be
  abbreviated as Fig., Sect. (or alternatively Sec.), Eq., Chap.\ and
  Ref.\ respectively, when they refer to a particular (numbered) item,
  except when they start a sentence. Table and Appendix are not
  abbreviated.  The plural form of abbreviation keeps the point after
  the s, \eg Figs.~1 and~2. Equations may be referred to either with 
  (``Eq.~(1)'') or without (``Eq.~1'') parentheses, 
  but it should be consistent within the paper.

\item Common abbreviations derived from Latin such as ``for example''
  (\eg), ``in other words'' (\ie), ``and so forth'' (\etc), ``and
  others'' (\etal), ``versus'' (\vs) can be used, with the typography
  shown, but not excessively; other more esoteric abbreviations should be avoided.
  

\item Units, material and particle names are usually lower case if
  spelled out, but often capitalised if abbreviated: amps (A), gauss
  (G), lead (Pb), silicon (Si), kaon (\kaon), but proton (\proton).

%\item The prefix for 1000 (k, \eg kV) should not be confused with
%  that used in computing (K, which strictly speaking denotes $2^{10}$,
%  \eg KB).

\item Counting numbers are usually written in words if they start a
  sentence or if they have a value of ten or below in descriptive
  text (\ie not including figure numbers such as ``Fig.\ 4'', or
  values followed by a unit such as ``4\,cm'').
  The word 'unity' can be useful to express the special meaning of
  the number one in expressions such as: 
``The BDT output takes values between zero and unity''.
% Numbers should not be
%  written as words if they by nature are real numbers that happen to
%  take an integer value, such as $\chisq/\mathrm{ndf} < 4$.

\item Numbers larger than 9999 have a comma (or a small space, but not both) between
  the multiples of thousand: \eg 10,000 or 12,345,678.  The decimal
  point is indicated with a point rather than a comma: \eg 3.141.

\item We apply the rounding rules of the
  PDG~\cite{PDG2016}. The basic rule states that if the three
  highest order digits of the uncertainty lie between 100 and 354, we round
  to two significant digits. If they lie between 355 and 949, we round
  to one significant digit. Finally, if they lie between 950 and 999,
  we round up and keep two significant digits. In all cases,
  the central value is given with a precision that matches that of the
  uncertainty. So, for example, the result $0.827 \pm 0.119$ should be
  written as $0.83\pm 0.12$, $0.827\pm 0.367$ should turn into
  $0.8\pm 0.4$, and $14.674\pm0.964$ becomes $14.7\pm1.0$.
 When writing numbers with uncertainty components from
  different sources, \ie statistical and systematic uncertainties, the rule
  applies to the uncertainty with the best precision, so $0.827\pm
  0.367\stat\pm 0.179\syst$ goes to $0.83\pm 0.37\stat\pm 0.18\syst$ and
  $8.943\pm 0.123\stat\pm 0.995\syst$ goes to $8.94\pm 0.12\stat\pm
  1.00\syst$.

\item When rounding numbers, it should be avoided to pad with zeroes
  at the end. So $51237 \pm 4561$ should be rounded as $(5.12 \pm 0.46)
  \times 10^4$ and not $51200 \pm 4600$.

\item When rounding numbers in a table, some variation of the rounding
  rules above may be required to achieve uniformity.

\item Hyphenation should be used where necessary to avoid ambiguity,
  but not excessively. For example: ``big-toothed fish'' (to indicate
  that big refers to the teeth, not to the fish), but ``big white
  fish''.  A compound modifier often requires hyphenation
  (\CP-violating observables, \bquark-hadron decays, final-state
  radiation, second-order polynomial), even if the same combination in
  an adjective-noun combination does not (direct \CP violation, heavy
  \bquark hadrons, charmless final state).  Adverb-adjective
  combinations are not hyphenated if the adverb ends with 'ly':
  oppositely charged pions, kinematically similar decay.  Words
  beginning with ``all-'', ``cross-'', ``ex-'' and ``self-'' are
  hyphenated \eg\ cross-section and cross-check. ``two-dimensional''
  is hyphenated. Words beginning with small prefixes (like ``anti'',
  ``bi'', ``co'', ``contra'', ``counter'', ``de'', ``extra'', "infra",
  "inter", "intra", "micro", "mid", ``mis'', "multi", "non", "over",
  "peri", "post", "pre", "pro", "proto", "pseudo", "re", "semi",
  "sub", "super", "supra", "trans", "tri", "ultra", "un", "under" and
  ``whole'') are single words and should not hyphenated
  \eg\ semileptonic, pseudorapidity, pseudoexperiment, multivariate,
  multidimensional, reweighted, preselection, nonresonant, nonzero,
  nonparametric, nonrelativistic, antiparticle,
  misreconstructed and misidentified.

\item Minus signs should be in a proper font ($-1$), not just hyphens
  (-1); this applies to figure labels as well as the body of the text.
  In Latex, use math mode (between \verb!$$!'s) or make a dash (``\verb!--!'').
  In ROOT, use \verb!#font[122]{-}! to get a normal-sized minus sign. 

\item Inverted commas (around a title, for example) should be a
  matching set of left- and right-handed pairs: ``Title''. The use of
  these should be avoided where possible.

\item Single symbols are preferred for variables in equations, \eg\
  \BF\ rather than BF for a branching fraction.

\item Parentheses are not usually required around a value and its
  uncertainty, before the unit, unless there is possible ambiguity: so
  $\dms = 20 \pm 2\invps$ does not need parentheses, whereas $f_d =
  (40 \pm 4)$\% or $x=(1.7\pm0.3)\times 10^{-6}$ does.
  The unit does not need to be repeated in
  expressions like $1.2 < E < 2.4\gev$.

\item The same number of decimal places should be given for all values
  in any one expression (\eg $5.20 < m_B < 5.34\gevcc$).

\item Apostrophes are best avoided for abbreviations: if the abbreviated term
  is capitalised or otherwise easily identified then the plural can simply add
  an s, otherwise it is best to rephrase: \eg HPDs, \pizs, pions, rather
  than HPD's, \piz's, $\pion$s.

\item Particle labels, decay descriptors and mathematical functions are not nouns, and need often to be followed by a noun. 
Thus ``background from $\Bd\to\pi^+\pi^-$ decays'' instead of ``background from $\Bd\to\pi^+\pi^-$'',
and ``the width of the Gaussian function'' instead of ``the width of the Gaussian''.

\item In equations with multidimensional integrations or differentiations, the differential terms should be separated by a thin space. 
Thus $\int f(x,y) dx\,dy$ instead $\int f(x,y) dxdy$ and
$\frac{d^2\Gamma}{dx\,dQ^2}$ instead of $\frac{d^2\Gamma}{dxdQ^2}$.
The d's are allowed in either roman or italic font, but should be consistent throughout the paper.


\end{enumerate}


==> wordcount.tex <==
\ProvidesFile{wordcount.tex}[2000/09/27 v1.5 Michael Downes]
% Copyright 2000 Michael John Downes
% This file has no restrictions on its use, distribution, or sale.
%
% If you run LaTeX on wordcount.tex it will prompt you for the name of a
% document to be counted. For most people, however, it will be more
% convenient to run the shell script wordcount.sh, giving the document
% name as the first argument. The comments in wordcount.sh
% give further information about the usage and limitations of this tool.

% The fundamental idea is to mark each character and interword space
% with a unique tag that will show up in TeX "showbox" output. Then
% arrange to make the output routine trigger a TeX overfull vbox message
% for the page box so that everything gets reported in the TeX log.
% Then run grep -c (or an equivalent text search utility, e.g., perl) on
% the log file to count the occurrences.
%
% In showbox output, a character is typically represented by a line of
% the form
%
%   ...\T1/cmr/m/n/10 e
%
% where "\T1/cmr/m/n/10" is the font name. We arrange things so that all
% characters are typeset in a font named "\3.08632". Furthermore, for
% interword spaces, which are normally represented in the output as
% something like
%
%   ...\glue 3.33333 plus 1.66666 minus 1.11111
%
% we use \spaceskip to ensure that it always appears as
%
%   ...\glue(\spaceskip) 3.08633 plus 9.0
%
% Then to count characters (including word spaces) we can
% grep for lines matching "3.0863", while to count words we
% count the number of lines in the log that match "3.08633" but not
% "3.08632".
%
% For an accurate count in multi-line paragraphs we also need
% to set rightskip to the flag value, since interword spaces are
% discarded at line breaks; and on the presumption that hyphenated
% compounds like "steady-state" should be counted as two words, we set
% \exhyphenpenalty to a value that ensures a line break at *every*
% explicit hyphen---then we will get a rightskip glue node between the
% two parts. (How about em-dashes? you may ask. Answer: it works all
% right, try it and see.)

\ifx\relax\?\def\wcQUIET{TT}\else\def\wcQUIET{TF}\fi

% We want accented letters to be represented by a single font char, to
% the extent possible:
\RequirePackage[T1]{fontenc}
\makeatletter
\thickmuskip=5.55555mu plus5.55555mu minus 2.22222mu
\let\@@thickmuskip\thickmuskip \newmuskip\thickmuskip
\let\@@spaceskip\spaceskip \xspaceskip=0pt
\newskip\@charfontname
% Ensure that these cannot be overridden.
\let\spaceskip\@charfontname \let\xspaceskip\spaceskip
\def\FreezeSpaces{%
  \setbox\z@\hbox{\mathsurround=\z@ $\mkern\@@thickmuskip$}%
  \@@spaceskip=\wd\z@ plus 9pt\relax
  % Setting rightskip to a slightly different value means that
  % end-of-line spaces can be distinguished if desired. (By default,
  % they are not.) Using fil units means there won't be any hyphenation
  % except for explicit hyphens.
  \dimen@\@@spaceskip \advance\dimen@ 1sp\relax
  \rightskip\z@ plus\strip@pt\dimen@ fil\relax
  % Prevent any further changes to \rightskip.
  \let\rightskip\spaceskip
  \@charfontname=\wd\z@ \advance\@charfontname -1sp\relax
  % Cancel all non-1000 sfcodes, which might otherwise affect the value
  % of inter-sentence spaces and keep them from being counted as
  % interword spaces.
  \def\do{\sfcode\fam\@m \advance\fam\@ne
    \ifnum\fam>\@cclv\expandafter\@gobble\fi \do
  }%
  \fam\z@ \do
  \let\frenchspacing\relax \let\nonfrenchspacing\relax
}
\def\DashPatch{%
  \exhyphenpenalty=-\@M \let\exhyphenpenalty\count@
  \hyphenpenalty\@M \let\hyphenpenalty\count@
  % LaTeX bug? Default definitions for these don't have \exhyphenpenalty
  % built in. Change them to just print a hyphen so that the penalties
  % will work.
  \def\textemdash{-}\def\textendash{-}%
}
% Here we set the font to ptmr8t (a T1 encoded font for which most
% people are likely to have a tfm file) and then make it difficult for
% the font to be changed ever again. We use two names for the font,
% \ptmr and \3.08632, the former being easier to use when resetting math
% fonts. The name that is defined last when TeX processes a document is
% the one that will be used in the log file.
\def\FreezeFont{%
  \expandafter\font
    \csname\strip@pt\@charfontname\endcsname
    =ptmr8t \relax
  \ptmr
  \check@mathfonts \let\check@mathfonts\relax
  \def\do{%
    \textfont\fam=\ptmr\scriptfont\fam=\ptmr\scriptscriptfont\fam=\ptmr
    \advance\fam\@ne \ifnum\fam<\sixt@@n \else\expandafter\@gobble\fi
    \do
  }%
  \fam=0 \do
}
\font\ptmr=ptmr8t \relax
\fontdimen22\ptmr=1sp % to permit use as math font 2
\let\selectfont\relax
\let\fontshape\@gobble \let\fontseries\@gobble \let\fontfamily\@gobble 
\let\fontencoding\@gobble \let\fontsize\@gobbletwo
\let\linespread\@gobble 
\let\try@load@fontshape\relax
\@namedef{U/msa/m/n}{}% disable special test in AMS documentclasses
\def\define@newfont{\expandafter\let\font@name=\ptmr}
\let\@@hfuzz\hfuzz \let\@@vfuzz\vfuzz
\newdimen\hfuzz \let\vfuzz\hfuzz
\def\QuietBoxes{%
  \@@hfuzz\maxdimen \@@vfuzz\maxdimen
}
\AtBeginDocument{\FreezeSpaces \FreezeFont \DashPatch \QuietBoxes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Halign patches
\def\ialign{\everycr{}\tabskip\@@spaceskip\halign} % initialized \halign
\def\extracolsep#1{\tabskip\@@spaceskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nofiles \let\makeindex\@empty % work-around for a natbib problem
% Seize control of the output routine to avoid extra clutter of dvi
% files. Handling \AtBeginDVI would take some extra work--for now I
% won't bother.
\def\showpagebox{%
  \showboxbreadth\maxdimen\showboxdepth99
  % This is a devious way of getting the box contents into the log file
  % without actually using \showbox (which typically results in a
  % nonzero exit code from the TeX run).
  \@@vfuzz\z@
  \setbox\z@\vbox to\z@{\box\@outputbox}%
  \setbox\z@\box\voidb@x
  \global \@colht \textheight
  \stepcounter{page}%
  \let\firstmark\botmark
}
\AtBeginDocument{\def\@outputpage{\showpagebox}}
\if\wcQUIET\else
\begingroup \def\msg^^J#1]^^J{\endgroup\message{#1]^^J^^J}}
\endlinechar=`\^^J \catcode`\ =12 \msg

The 'wordcount' utility provides a way of estimating the number of
words in a LaTeX document.

[Warning: The counting method uses a large log file as an intermediate
step. If your disk space is extremely low the counting process
may end prematurely for lack of space.]

\fi

% \typein has extraneous blank lines and slightly idiosyncratic prompt.
\begingroup \endlinechar=-1
\message{File name [press RETURN to cancel]: }
\def\do{%
  \let\do\@makeother \dospecials
  \global\read-1 to\wcFileName
  \endgroup
}
\do

\ifx\@empty\wcFileName
  \typeout{No file name given; quitting.}\expandafter\@@end\fi

\expandafter\filename@parse\expandafter{\wcFileName}
\edef\jobname{\filename@base}

\if\wcQUIET
  \message{\wcFileName}
\else
\typeout{^^JTo get a count of characters, run^^J^^J \space
%
  grep -c '3[.]0863[23]' wordcount.log^^J^^J%
%
or equivalent when processing is finished.^^J%
}
\fi

\typeout{Processing \wcFileName...^^J}

\IfFileExists{\wcFileName}{\batchmode}{\nonstopmode}
\edef\@tempa{\noexpand\makeatother
  \noexpand\input{\wcFileName}\noexpand\stop
}
\@tempa

